CARLA: An Open Urban Driving Simulator

We introduce CARLA, an open-source simulator for autonomous driving research. CARLA has been developed from the ground up to support development, training, and validation of autonomous urban driving systems. In addition to open-source code and protocols, CARLA provides open digital assets (urban layouts, buildings, vehicles) that were created for this purpose and can be used freely. The simulation platform supports flexible specification of sensor suites and environmental conditions. We use CARLA to study the performance of three approaches to autonomous driving: a classic modular pipeline, an end-to-end model trained via imitation learning, and an end-to-end model trained via reinforcement learning. The approaches are evaluated in controlled scenarios of increasing difficulty, and their performance is examined via metrics provided by CARLA, illustrating the platform's utility for autonomous driving research. The supplementary video can be viewed at https://youtu.be/Hp8Dz-Zek2E

==> tex/background.tex <==
\section{Related Work}
\label{sec:background}

Raw sensor data together with ground truth and/or privileged information is critical for designing, training and validating autonomous agents. Simulators allow to produce all this information in an efficient manner and can lead to the generation of groundbreaking new knowledge.

Pursuing this idea, different works have focused on the use and creation of simulated environments to produce synthetic data for developing algorithms to obtain visual cues such as optical flow~\citep{Butler:2012, Mayer:2016} and disparity from stereo \citep{Haeusler:2013}. Other works proposed the use of synthetic data to develop scene understanding modules for indoor scenes~\citep{Handa:2016} and for driving scenarios~\citep{Haltakov:2013, Ros:2016, Gaidon:2016, Shafaei:2016, Richter:2016}; even to learn unwritten common sense~\citep{Vedantam:2015} or classifying videos according to actions \citep{DeSouza:2017}. Since the ultimate goal of autonomous agents is, indeed, operating within a desired environment, other works focused on training the agents by in simulation rather than only producing datasets. Examples of these are used to learn physical intuition in a simple blocks world \citep{Lerer:2016}, or to perform interaction with static objects in photo-realistic indoor scenarios\citep{Zhu:2016}. For the specific domain of autonomous driving, TORCS \citep{Wymann2014torcs} has been used for learning mediated driving representations  for autonomous navigation\citep{Chen:2015}. However, in most of the cases the available open frameworks are very constrained  in terms of scenario complexity and assets variability, limiting the scope of the study. The research community found a more challenging and complex alternative in AAA video games, such as GTA-V, which can be used for urban driving simulation, not only to produce datasets such as in \citep{Richter:2016}, but also to perform in-game training~\citep{Kinsley:2016}. However, these engines are not open source and, therefore, their usability for simulation purposes is restricted and recently it has even claimed to be illegal.

CARLA brings the best qualities of the previous tools. Firstly, it is totally open source, both the code and also all the 3D assets, including towns, vehicles, pedestrians, etc. It can generate synthetic datasets with ground truth including images with pixel-wise semantic classes, depth, etc. It also provides privileged information such as GPS-like information of the vehicle, speed, 3D acceleration vector, timestamps (in game and OS), degree of invasion in both opposite lanes and sidewalks, collision strength segregated per vehicles, pedestrians and others (infrastructure, houses, trees, rocks), etc. But most importantly, CARLA is an urban driving simulator that allows autonomous agents to drive within urban scenarios for learning to act and assessing their capabilities. In this sense, CARLA is a clear step forward in simulation, addressing urban scenarios in a highly realistic way, both in terms of graphics and fidelity. CARLA's focus is set on challenging situations,  where the layout of the scene is complex (e.g.,  intersections with traffic signs, sidewalks, buildings, etc.) and strong interaction and negotiation with other vehicles and pedestrians is required.

%testing their performance, and carrying out ablative analyses over the training and testing variables.
%Collecting the raw data is itself time consuming ({\eg}, a car driving around the world acquiring images) but, even worse, providing the corresponding ground truth is really difficult to scale ({\eg}, pixel-wise manual labeling of images may take even 90 minutes per image), difficult to measure ({\eg}, know how much the ego car is invading the opposite lane or a sidewalk during training/testing runs), or even impossible ({\eg}, obtaining accurate depth information from a single image). This data curse is even more demanding when we rely on deep learning models as required for perception and control tasks. A promising approach to tackle this problem consists in the use of
%Virtual environments allow to produce all this information in an efficient manner and even running informative simulations.

%In \citep{Butler:2012} it is proposed the SINTEL synthetic datasets for evaluating optical flow algorithms in challenging conditions. In \citep{Mayer:2016} a large dataset of synthetic images is proposed for training deep estimators of disparity, optical flow, and scene flow. In \citep{Haeusler:2013}, a synthetic dataset is used for evaluating stereo-based disparity estimators. Beyond, low level vision cues, in \citep{Handa:2016} understanding of indoor scenes is based on training models for semantic segmentation using synthetically generated RGB-D images with the required ground truth.  ....

%Following this approach, different works focused on the use and creation of simulated environments to produce synthetic data for developing algorithms to obtain visual cues such as optical flow~\citep{Butler:2012, Mayer:2016} and disparity from stereo \citep{Haeusler:2013}. Other works proposed the use of synthetic data to develop scene understanding modules for indoor scenes~\citep{Handa:2016} and for driving scenarios~\citep{Haltakov:2013, Ros:2016, Gaidon:2016, Shafaei:2016, Richter:2016}; even to learn unwritten common sense~\citep{Vedantam:2015} or classifying videos according to actions \citep{DeSouza:2017}. Since the ultimate goal of autonomous agents is, indeed, operating within a desired environment, other works focused on training the agents by in simulation rather than only producing datasets. Examples of these are used to learn physical intuition in a simple blocks world \citep{Lerer:2016}, or to perform interaction with static objects in photo-realistic indoor scenarios\citep{Zhu:2016}. For the specific domain of autonomous driving, TORCS \citep{Wymann2014torcs} has been used for learning mediated driving representations  for autonomous navigation\citep{Chen:2015}.
%
%%Beyond these works, CARLA is an urban driving simulator that not only allows to generate synthetic datasets with ground truth ({\eg} images with pixel-wise semantic classes and depth), but also allows AI agents to drive within the created urban scenarios for learning to act and assessing their capabilities.
%CARLA is a clear step forward because it addresses urban scenarios, where dealing with other cars as in racing is required, but we must take also into account pedestrians, road intersections, traffic rules, sidewalks, houses, etc. Moreover, CARLA presents a higher degree of photo-realism than TORCS and allows simulations under different lighting and weather conditions.
%
%%In addition,
%Finally, we would like to remark that there are videogames such as GTA-V which can be used for urban driving simulation, not only for producing datasets such as in \citep{Richter:2016}. However, they are not open source and, therefore, their usability for simulation purposes is restricted. In contrast, CARLA is totally open source, not only in terms of the code but also including the current towns and the assets used for building them. CARLA has been built for the AI vehicle easily accessing different signals useful for its training and testing. For instance, GPS-like information of the AI vehicle, speed, 3D acceleration vector, timestamps (in game and OS), degree of invasion in both opposite lanes and sidewalks, collision strength segregated per vehicles, pedestrians and others (infrastructure, houses, trees, rocks), etc.

%Finally, in this paper we not only present CARLA as simulator, but also show quantitatively how useful CARLA is for training AI vehicles using two different paradigms, namely end-to-end driver imitation learning and the integration of separated modules for perception and maneuver control.

